Event-B/SLP

We show how the event-based notation offered by Event-B may be augmented by algorithmic modelling constructs without disrupting the refinement-based development process.

==> misc.tex <==
\subsection{\KASSERT statement}

\EXAMPLE{
	s \bcmeq s \cup \{e\} \KSEQ
	s \bcmeq s \setminus \{g\} \KSEQ
	t \bcmin s
}

\EXAMPLE{
	s \bcmeq s \cup \{e\} \KSEQ
	s \bcmeq s \setminus \{g\} \KSEQ
	\KASSERT s \neq \emptyset  \KSEQ
	t \bcmin s
}

\EXAMPLE{
	s \bcmeq s \cup \{e\} \KSEQ
	\KASSERT s \setminus \{g\} \neq \emptyset  \KSEQ
	s \bcmeq s \setminus \{g\} \KSEQ
	\KASSERT s \neq \emptyset  \KSEQ
	t \bcmin s
}

\EXAMPLE{
	s \bcmeq s \cup \{e\} \KSEQ
	\KASSERT s \cup \{e\} \neq \{g\}  \KSEQ \\
	\KASSERT s \setminus \{g\} \neq \emptyset  \KSEQ
	s \bcmeq s \setminus \{g\} \KSEQ 
	\KASSERT s \neq \emptyset  \KSEQ
	t \bcmin s
}


There is a difference between a composition of a assertion via sequential composition operator $\KWD{;}$ and a composite assert. The following makes 

\EXAMPLE{
	s \bcmeq s \cup \{e\} \KSEQ
	\KASSERT e \in s \KSEQ
 	\KASSERT s \neq \emptyset
}


\EXAMPLE{
	\HYP \vdash e \in s \cup \{e\} \\
	\HYP, e \in s \vdash s \neq \emptyset \\
}


\EXAMPLE{
	s \bcmeq s \cup \{e\} \KSEQ
	\KASSERT e \in s ~\KASSERT e \neq \emptyset
}


\EXAMPLE{
	\HYP \vdash e \in s \cup \{e\} \land s \neq \emptyset \\
}



$$
\begin{array}{rcl}
\RW{\KSTOP} & := & \emptyset \\
\RW{\KASSERT~ p } & := & \emptyset \\
\RW{a \KSEQ b} & := & \RW{a} \cup \RW{b} \\
\RW{u \bcmeq E(v)} & := & u \\
\RW{u \bcmin E(v)} & := & u \\
\RW{u \bcmsuch E(v, v')} & := & u \\
\RW{
\KIF~ c_0 ~ \KTHEN~ b_0 \\
\KELSEIF~ c_1 \KTHEN ~ b_1 \\
\dots \\
\KELSEIF~ c_k \KTHEN ~ b_k \\
\KELSE~ b_e~ \KEND
}
& := & \bigcup_{j \in 0 \upto k} \RW{b_j}
 \\

\RW{
\KWHILE ~ c \\
\KINV ~ I \\
\KVAR ~ V \\
\KTHEN~ b ~ \KEND ~
}
& := &
\RW{b} \\

\RW{
\KBEGIN \\
\KINV ~ I\\
b  \\
\KEND
}
& := &
\RW{b} \cap v \\
\end{array}
$$

